Self-Supervised Joint Encoding of Motion and Appearance for First Person Action Recognition

Wearable cameras are becoming more and more popular in several applications, increasing the interest of the research community in developing approaches for recognizing actions from the first-person point of view. An open challenge in egocentric action recognition is that videos lack detailed information about the main actor's pose and thus tend to record only parts of the movement when focusing on manipulation tasks. Thus, the amount of information about the action itself is limited, making crucial the understanding of the manipulated objects and their context. Many previous works addressed this issue with two-stream architectures, where one stream is dedicated to modeling the appearance of objects involved in the action, and another to extracting motion features from optical flow. In this paper, we argue that learning features jointly from these two information channels is beneficial to capture the spatio-temporal correlations between the two better. To this end, we propose a single stream architecture able to do so, thanks to the addition of a self-supervised block that uses a pretext motion prediction task to intertwine motion and appearance knowledge. Experiments on several publicly available databases show the power of our approach.

==> soaOLD.tex <==
\section{Related works}
\label{sec:soa}

\textbf{First Person Action Recognition.}
Deep learning approaches are the state of the art in FPAR


\andrea{Questo SOA e' vecchio, bisogna fare una passata sui nuovi lavori (CVPR,ICCV, etc...)}
The literature on first-person action recognition has long acknowledged that the motion of the hands, the appearance of the objects being used, and the interplay of these two components are the most critical characteristics to extract from raw data \cite{degeest2016,pirsiavash2012,ghirshick2015}.
This approach has moved from handcrafted features-based works to the deep learning wave \cite{ma2016,Li_2018_ECCV,sudhakaran2018attention}, providing researchers with powerful and effective models for encoding appearance. 
However, when it comes to action recognition, these methods rely on simple aggregation of frame-wise decisions, and they completely neglect the temporal relationships and the dynamics between frames.
%Still, learning the temporal features from static images is still challenging and 
Several approaches exploit Convolutional Long Short-Term Memory (ConvLSTM) networks to tackle this issue \cite{Sudhakaran_2019_CVPR,sudhakaran2018attention}. ConvLSTMs attempt to model the temporal dependencies between frames by taking into account within-frame spatial correlations too. However, it is still not clear if the temporal features extracted by these networks are as effective as those obtained leveraging explicit optical flow data in capturing complex and unsteady motion dynamics.

\andrea{qui possiamo dire che i 2stream usano o conv2d o conv3d}

To this end, many recent deep learning methods for action recognition follow the two-stream approach \cite{Simonyan2014,spriggs2017,mahmud2017,sudhakaran2018attention}. This method addresses the two tasks of recognition from motion and recognition from appearance with different networks that are either combined with late fusion, i.e., before the classification step, or at the decision level. Furthermore, while the appearance stream analyzes individual RGB frames, the motion stream usually processes a short sequence of stacked adjacent flow frames that, typically, have no one-to-one relation with the RGB input. This lack of correlation between the spatial and temporal information processed limits the network capabilities of extracting complex motion dynamics in long video segments. 

Recent works attempted to \andrea{strengthen} the temporal aspects of videos using attention mechanisms \cite{Zhang2018,sudhakaran2018attention,Sudhakaran_2019_CVPR} to find the most informative parts through single images (spatial attention) or video segments (temporal attention). These approaches are generally cast within a two-stream framework. Although they have shown a reasonable degree of success, the resulting architectures tend to increase their complexity and often need to be trained in two stages or more.  

\andrea{A possible alternative consist in jointly modelling appearance and motion into a single stream. [aggiungere discussione].
(Dance with flow) propose to combine optical flow and RGB into a single stream, reducing the computational cost of two-stream approaches and facilitating end-to-end training. However, it still requires the use of optical flow at test time.
}

\mirco{
\textbf{Joint Appearance and Motion Stream.}}
\begin{itemize}
\item Three main challenges related to video understanding concern: the spatial image features representation, the temporal information representation, and model/computation complexity.
\item Both the more common approach in the literature, two-stream and 3D CNN [cit lavori di Zisserman], although the high performances achieved, they introduce a high model/computation complexity.
\item Recently works try to avoid this problem in different ways.
\item (Dance with flow) propose a single stream method for action detection, unfortunately, it still requires the computation of optical flow for both the training and test data,  which is computationally expensive.
\item Other works [ref1, ref2] have attempted to jointly model appearance and motion into a single stream, introducing modules designed to better exploit the temporal information, but leading to complex architectures.
\item (Mars) attempts to hallucinate the optical flow information in order to avoid to compute it a test time. It is very important for recognizing actions in an online scenario.
\item We propose a method single stream that a test time use only the RGB data
\end{itemize}
\mirco{forse potremmo aggiungere anche qualche referenza a quelli che provano a stimare l'optical flow come task ausiliario, che comuqneu presentato delle strutture pesanti}

\textbf{Motion-based Self-Supervised Tasks.}
Self-Supervised Learning \cite{SSLsurvey} has been recently introduced for learning visual features from unlabeled data. The choice of an auxiliary task that does not require human annotation of the data enables the network to encode a knowledge that proves beneficial as initialization when solving a classification problem on related data. Different authors have proposed several auxiliary tasks, either relying on original visual cues (e.g., translation, scaling, rotation \cite{gidaris2018unsupervised,NIPS2014_geometric}, clustering  \cite{caron2018deep}, inpainting \cite{pathakCVPR16context} and colorization), on information extracted from image patches \cite{learningtocount,NorooziF16,Noroozi_2018_CVPR}, or regularities introduced by the temporal dimension in videos \cite{Wang_UnsupICCV2015,SSLvideo}.
The use of motion cues in self-supervised learning has been first proposed in \cite{Pathak2017}, where authors trained a convolutional network to segment a static frame (in an unsupervised way) using motion data obtained from videos. Optical flow cues had been exploited in \cite{HoWRC15}, to learn the visual appearance of obstacles in a Micro Air Vehicle landing environment. Also \cite{Lee2015} used a self-supervised motion segmentation task applied to monoscopic visual odometry and ground areas labeling.
Instead, \cite{Mahendran2018} \quotes{transfer} optical flow information to pixel embeddings so that their difference matches that between optical flow vectors of the same pixels. 
Finally, \cite{wang2019selfsupervised} regresses the spatial and temporal statistics of motion and appearance to learn spatio-temporal features for video representation. The main difference with our approach is that \cite{wang2019selfsupervised} leverages 3D convolutions that, working on volumes, already include implicit motion information clues (beyond that instilled by the auxiliary task) that we can not benefit from in our method, as we use sparse and individual images as input. 
\andrea{CItrae per il movimento l'articolo dima damen (che usa OF per fare domain adaptation)}




% \textbf{Learning to Recognize with Self-Supervised Tasks.}
% \andrea{Maybe, Motion-based Self-Supervised Tasks. Then we can get rid of the first part (summarizing it in a short paragraph)}
% Self-Supervised Learning \cite{SSLsurvey} has been recently introduced for learning visual features from unlabeled data. The choice of an auxiliary task that does not require human annotation of the data enables the network to encode %into the first layers 
% a knowledge that proves beneficial as initialization when solving a classification problem on related data. 
% The transfer of the model learned by solving the self-supervised task to a downstream classification net has proved to be useful in many contexts. Different authors have proposed several auxiliary tasks roughly organized into three main groups. 
% The first relies only on original visual cues and involves either the whole image with geometric transformations (e.g., translation, scaling, rotation \cite{gidaris2018unsupervised,NIPS2014_geometric}), clustering  \cite{caron2018deep}, inpainting \cite{pathakCVPR16context} and colorization \cite{zhang2016colorful}, or considers image patches focusing on their equivariance (learning to count \cite{learningtocount}) and relative position (solving jigsaw puzzles \cite{NorooziF16,Noroozi_2018_CVPR}).
% The second group uses real or synthetic external sensory information. This approach is popular for multi-cue problems (visual-to-audio \cite{audiovisual}, RGB-to-depth \cite{ren-cvpr2018}) and in robotics \cite{grasp2vec,visiontouch}.
% Finally, the third group relies on video and the regularities introduced by the temporal dimension \cite{Wang_UnsupICCV2015,SSLvideo}.
% The use of motion cues in self-supervised learning has been first proposed in \cite{Pathak2017}, where authors trained a convolutional network to segment a static frame (in an unsupervised way) using motion data obtained from videos. Optical flow cues had been exploited in \cite{HoWRC15}, to learn the visual appearance of obstacles in a Micro Air Vehicle landing environment. Also \cite{Lee2015} used a self-supervised motion segmentation task applied to monoscopic visual odometry and ground areas labeling.
% Instead, \cite{Mahendran2018} \quotes{transfer} optical flow information to pixel embeddings so that their difference matches the difference between optical flow vectors of the same pixels. 
% Finally, \cite{wang2019selfsupervised} regresses the spatial and temporal statistics of motion and appearance to learn spatio-temporal features for video representation. The main difference with our approach is that \cite{wang2019selfsupervised} leverages 3D convolutions that, working on volumes, already include implicit motion information clues (beyond that instilled by the auxiliary task) that we can not benefit from in our method, as we use sparse and individual images as input. 
% \andrea{CItrae per il movimento l'articolo dima damen (che usa OF per fare domain adaptation)}

%Third, as acknowledged by the Reviewer, the amount of camera motion and shake in egocentric videos is usually much more significant than what is observable in third-person datasets. Thus, a simple derivative of the dense optical flow is unlikely to be able to suppress the influence of such camera movements entirely.

%Concluding, we underline again that, to the best of our knowledge, the specific self-supervised auxiliary task (motion segmentation) is used here for the first time in the area of action recognition.

%4) another one to check is \cite{Zhan2019} 



%\subsection{Relation to State-of-the-Art Alternatives}
%\textbf{Comparison with BMVC \cite{sudhakaran2018attention}} The main advantages of our approach are the following:

%\begin{itemize}
 %   \item it analyzes a smaller amount of frames, and, thus, it is computationally lighter
  %  \item for the same reason, it guarantees faster training times 
   % \item the whole network can be trained end-to-end and in a single stage (on the contrary \cite{sudhakaran2018attention} requires at least three stages: first, train the flow branch to get the LSTA bias initialization, then, train in two stages the RGB branch)
%\end{itemize}





